Target Tracking Using the Invariant Extended Kalman Filter with Numerical Differentiation for Estimating Curvature and Torsion

The goal of target tracking is to estimate target position, velocity, and acceleration in real time using position data. This paper introduces a novel target-tracking technique that uses adaptive input and state estimation (AISE) for real-time numerical differentiation to estimate velocity, acceleration, and jerk from position data. These estimates are used to model the target motion within the Frenet-Serret (FS) frame. By representing the model in SE(3), the position and velocity are estimated using the invariant extended Kalman filter (IEKF). The proposed method, called FS-IEKF-AISE, is illustrated by numerical examples and compared to prior techniques.

==> OLD_Files/zDiscussions.tex <==


This file is a report on the various DT absolute stability results.

Here is what Prof Haddad sent me:


The status for the DT case is a bit of a mess. I looked into this problem very carefully back in the 90’s. I have collected all of the key results in my NL book for the DT absolute stability problem; see Problems 13.24, 13.25, 13.26, 13.27 (which is the DT circle criterion), and Problem 13.28 (the Szego criterion, which is the DT analog of the Popov criterion).

DDDDDD  you have these pages


 
In our paper (the one that you sent me) we do talk about the (multivariable) DT circle criterion and give a proof of the result. See Section 5 of the paper.

DDDDD  this is the paper:  EXPLICIT CONSTRUCTION OF QUADRATIC LYAPUNOV
FUNCTIONS FOR THE SMALL GAIN, POSITIVITY,
CIRCLE, AND POPOV THEOREMS AND THEIR
APPLICATION TO ROBUST STABILITY.
PART II: DISCRETE-TIME THEORY




There is also the Tsypkin criterion, which Vikram and I extended to the multivariable case (see Reference 62 on my website).

DDDD  Pls obtain




Also see the relevant References 44 and 54 in my website. In our Automatica paper (Ref. 44) see Theorem 4.3. And in my IJC paper with Vikram (Ref. 54) we have all of the key DT absolute stability results---the DT circle criterion is a special case.

DDDD  pls check


Finally, also see:  Wu, S. H., 'A circle stability criteria for a class of discrete system', IEEE Trans. Autom. Contr., AC-12, pp. 114-115, (1967).

DDDD  pls get

DDD  also search thanks


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


here


Hiu Juan

couple things

first, the 2-PCAC controller is working well, thanks for the suggestion!




JJJ: The theorems we cite only mention global asymptotic stability


right.  Do we define absolute stability in the paper?  OK, then perhaps we should ......follow me...........

No, we definitely should.


OK, this is shaping up

let me explain how you might do DOA

1.  You run pcac for xxx steps

2.  At step xxx you estimate the DOA.  The way to do this is how REza does it:

a.  you grid the plane
b.  if you believe you have convergence, you plot a green square.  If not, a red square.  I will share Rezas paper so you can see how he did it 
c.  Then you RERUN pcac from a LARGER initial condition.
d.  Yoiu check DOA again.  Do all green stay green?  that's critical
e.  If a red square now converges, use blue.  the blue squares mean that the DOA got larger.
f.  now that I think of it, you might just need to make say 4 plots

Plot 1.  green/red for one IC
Plot 2.  green/red for ANOTHER IC
etc

is it clear?

**************see figure 7 in rezas paper



Wait, when you say PCAC you mean the converged system?

I only need 1 plot. I get the set of thetas and the gain K at the end of the pcac run, I ran the converged system for a grid of initial conditions and the I plot all trajectories in a k vs log_10 (|y_k|) plot, which will show whether the trajectories converge.

hmmmmmm  what agbout initial conditions?  

They correspond to the grid I mentioned

will this show that the DOA gets larger?

Wait, larger relative to the open-loop?

no, we want to know if the DOA gets larger as the initial condition gets larger----take SOME x_0 and multiply it by 2, 5, 10 etc and see if DOA gets larger----this might be tricky-----we dont know yet what will happen




It doesn't get larger, the original DOA seems to be already global in the example I ran. 


The convergent PCAC system does not meet the absolute stability criteria, but I cannot find initial conditions that don't converge 

got it.  ok, then this is NOT what I thought------we need to do this:


1.  We need to convince the reader that after xxx steps, the DOA is VERY LARGE.  how can you show this???????

k vs log_10 (|y_k|) for initial conditions in the order of 10^8. It converges, I can plot it.

how will you choose ICs?

[-10000000: 100000: 1000000] X [-1000000: 100000: 10000000]. I plot all log_10 (|y_k|) trajectories

 









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hi Juan

I changed

alpha_cc

to

alpha_CC

this is more consistent with CC1 and also TC1

sorry you have to modify the figures

JJ You sure? It looks a bit awkward with CC instead of cc

I know 

also:

$1 - \alpha_{N, k}$-----------------something is wrong with this notation, it should be alpha_TC but TC is missing something is cvonfusing me

I had it as alpha_tc, it should be $\alpha_{TC, N, k},$ right? This is only an issue in the figure captions


$\alpha_{TC, N, k},$<-----------------------YES use this

I'll make the corrections to all figure and captions then, it won't take me long


I know CC and TC look awkward but we need to use T not t since it is a name

I am running out of time-----------pls do as much as you vcan-------we will finish when we meet on Tuesday no matter what


Anything else I should check other than the alpha and beta notation?

no that is all I can think of

notice I changed DMISB to DISB and other minr changes

Got it, it shouldn't be an issue. I'll check the whole document then.

I made a lot of minor wording changes mostly to streamline

ok, good

what can you do on the PID paper?


Include the PID formulations and the new DD formulation, as well as the architecture considered in the paper.


ok, good!  I will write the intro on Wed and we will go over it tuesday ok?  Thanks  We still have a LOT to do!


You will write the intro after we meet then, got it.

right I am out of time until Tuesday evening


Don't worry, I'll work on it and put it in good shape.


check all alpha and beta in figure captions-------there are errors thanks

Will do

Thank you!!!  ok bye for now and I appreciate a great effort at being super productive!!!!!  thanks ok!


Don't worry about it, ttyl!







